Asking for Knowledge: Training RL Agents to Query External Knowledge Using Language

To solve difficult tasks, humans ask questions to acquire knowledge from external sources. In contrast, classical reinforcement learning agents lack such an ability and often resort to exploratory behavior. This is exacerbated as few present-day environments support querying for knowledge. In order to study how agents can be taught to query external knowledge via language, we first introduce two new environments: the grid-world-based Q-BabyAI and the text-based Q-TextWorld. In addition to physical interactions, an agent can query an external knowledge source specialized for these environments to gather information. Second, we propose the "Asking for Knowledge" (AFK) agent, which learns to generate language commands to query for meaningful knowledge that helps solve the tasks. AFK leverages a non-parametric memory, a pointer mechanism and an episodic exploration bonus to tackle (1) irrelevant information, (2) a large query language space, (3) delayed reward for making meaningful queries. Extensive experiments demonstrate that the AFK agent outperforms recent baselines on the challenging Q-BabyAI and Q-TextWorld environments.

==> back.tex <==
% !TEX root = main.tex
\section{Background}
\label{sec:background}




\subsection{Reinforcement Learning}
%\textbf{Reinforcement Learning.}
Reinforcement learning considers an agent interacting with an environment and collecting reward over discrete time. The environment is formalized by a partially observable Markov Decision Process (POMDP)~\cite{SuttonRL}. Formally, a POMDP is defined by a tuple $(\cS, {\cA}, \cZ, {\cT}, \cO,  R, \gamma, H)$. $\cS$ is the state space. {\cal A} is the action space. $\cZ$ is the observation space. At each time step $t$, the agent receives an observation $o_t \in \cZ$ following the observation function $\cO: \cS \rightarrow \cZ$ and selects an action $a_t \in \cA$. The transition function $\cT$ maps the action $a_t$ and the current state $s_t$ to a distribution over the next state $s_{t+1}$, \ie $\cT: \cS \times \cA \rightarrow \Delta(\cS)$. The agent receives a real-valued reward $r_t$ according to a reward function $R: \cS \times \cA \rightarrow \cR$. The agent's goal is to maximize the return $\sum_{t=0}^{H} \gamma^t r_t$, where $\gamma$ is the discount factor and $H$ is the horizon. 

\subsection{Query Environment}
%\textbf{Query Environment.} 
In a query environment, the agent receives not only observation from the environment but also a response from the knowledge source if it made a query. Therefore, the observation space $\cZ$ can be decomposed as $\cZ = \cZ_{\text{env}} \times \cZ_{q}$, where $\cZ_{\text{env}}$ is the environment observation space.  $\cZ_{q}$ is the response space. 

In addition, at each times step, the agent could either takes a physical action or make a query. Therefore, we denote the action space as  $\cA = \cA_{\text{phy}} \bigcup \cA_{q}$, where $\cA_{\text{phy}}$ is the physical action space supported by common BabyAI and TextWorld environment. $\cA_{q}$ is the query action space. 

\label{subsec:back_rl}



==> fig_tasks.tex <==
% !TEX root = main.tex


\begin{figure*}[t!]
\centering
\includegraphics[width=1.0\textwidth]{figures/task_examples.pdf}
\caption{Querying interactions in \qbai and \qtw. We omit standard physical interactions due to space limitation.}
\vspace{-0.0cm}
\label{fig:tasks}
\end{figure*}


==> tb_abl.tex <==
% !TEX root = main.tex


\begin{table*}[t] 
\centering
\begin{center}
{
\begin{tabular}{c|cccccccc}
\specialrule{.15em}{.05em}{.05em} 
                        & \multicolumn{2}{c}{\makecell{AFK w/o \\ Notebook}} & \multicolumn{2}{c}{\makecell{AFK w/o \\ Pointer Mechanism} } &  
                      \multicolumn{2}{c}{\makecell{AFK w/o \\ Episodic Exploration} }  &  
                      \multicolumn{2}{c}{\makecell{AFK \\(Ours)} }  
                       \\ \toprule\toprule
                      		Task		         & Succ.             & Eps. Len.             & Succ.             & Eps. Len.           & Succ. & Eps.  Len.   & Succ. & Eps. Len.        \\ \hline

\makecell{\sclub}    &   50.0$\pm$0.8  & 	5.67$\pm$0.1	& 49.4$\pm$0.7  & 	6.4$\pm$0.1  &	49.8$\pm$0.7 & 6.01$\pm$0.07 & \bf{100.0$\pm$0.0}   & \bf{10.8$\pm$0.1}        \\
\makecell{\sspade}    &   99.1$\pm$0.2  & 	10.1$\pm$0.0	& 100.0$\pm$0.0  & 	10.5$\pm$0.1  &	93.8$\pm$0.7 & 9.7$\pm$0.1 & \bf{100.0$\pm$0.0}   & \bf{10.4$\pm$0.0}        \\
\makecell{\sdiamond}    &   99.2$\pm$0.4  & 	27.8$\pm$1.9	& 99.7$\pm$0.2  & 	21.3$\pm$1.0  &	99.3$\pm$0.2 & 27.3$\pm$1.1 & \bf{99.9$\pm$0.0}   & \bf{16.8$\pm$6.7}        \\
\makecell{\sheart}    &   85.1$\pm$1.0  & 	37.9$\pm$1.2	& 100.0$\pm$0.0  & 	20.6$\pm$0.18  &	77.8$\pm$0.7 & 42.8$\pm$0.8 & \bf{100.0$\pm$0.0}   & \bf{20.6$\pm$0.2}        \\
\makecell{\sclub\sheart}    & 48.5$\pm$1.9  & 26.7$\pm$0.6	& 90.5$\pm$1.4  & 	32.8$\pm$0.9  &	50.0$\pm$1.8 & 26.6$\pm$0.7 & \bf{95.8$\pm$0.5}   & \bf{32.3$\pm$0.6}        \\
\bottomrule
\makecell{Comp.}    &  0.73   & 	& 0.84 &  &	0.79 &  & 1.0   & 1.0        \\





\end{tabular}
}
\caption{Ablation Study. \sclub: \oib, \sspade: \danger, \sdiamond: \gtfav, \sheart: \od.}
\label{tb:abl}
\end{center}
\end{table*}

==> tb_all_info_distractor.tex <==
% !TEX root = main.tex


\begin{table*}[t] 

\begin{center}
{
\begin{tabular}{c|cccccc}
\specialrule{.15em}{.05em}{.05em} 
                       & \multicolumn{2}{c}{\makecell{All Info. w/ Distractors} }& \multicolumn{2}{c}{\makecell{All Info. w/o Distractors} } &  
                      \multicolumn{2}{c}{\makecell{AFK (Ours)} }  \\
                      \toprule\toprule
                      		Task		       & Succ. ($\%$)            & Eps. Len.             & Succ. ($\%$)           & Eps. Len.     & Succ. ($\%$)           & Eps. Len.                \\ \hline

\multirow{1}{*}{\makecell{Object  in Box}}     
& $\pm$ &	$\pm$    &          $\pm$ &	$\pm$	& \bf{$\pm$} & \bf{$\pm$}    \\



\multirow{1}{*}{Danger}     
& $\pm$ &	$\pm$    &      $\pm$& $\pm$ &	\bf{$\pm$} & \bf{$\pm$}               \\


\multirow{1}{*}{\makecell{Go to  Favorite}}
& $\pm$ &	$\pm$    &     $\pm$ &	$\pm$ &	\bf{$\pm$} & \bf{$\pm$}               \\
 

\multirow{1}{*}{\makecell{Open Door}}     
& $\pm$ &	$\pm$    &      $\pm$ &	$\pm$ &	\bf{$\pm$} & \bf{$\pm$}               \\


\end{tabular}
}
\caption{.}
\label{tb:oracle}
\end{center}
\end{table*}

==> tb_all_res.tex <==
% !TEX root = main.tex


\begin{table*}[t] 

\begin{center}
{
\begin{tabular}{c|c|c|c|c|cccccc}
\specialrule{.15em}{.05em}{.05em} 
                      & \multicolumn{4}{c}{\makecell{Tasks} } & \multicolumn{2}{c}{\makecell{No Query}} & \multicolumn{2}{c}{\makecell{Query Baseline} }  & \multicolumn{2}{c}{\makecell{AFK (Ours)} } \\ \toprule\toprule
                      				& \makecell{Object \\ in Box} & \makecell{Danger} & \makecell{Go to \\ Favorite}  &   \makecell{Open \\ Door}      & Succ.($\%$)             & Eps. Len.             & Succ.($\%$)              & Eps. Len.           & Succ.($\%$)              & Eps. Len.         \\ \hline

\multirow{4}{*}{Lv. 1}     
& V & & &    &   50.5$\pm$0.6      & 5.9$\pm$0.1	&49.8$\pm$1.1 &6.0$\pm$0.1	 &	\bf{100.0$\pm$0.0} &  \bf{10.8$\pm$0.1}              \\
 & &V & &      &  68.3$\pm$0.8     &	8.2$\pm$0.0	&73.8$\pm$0.9 &8.3$\pm$0.1	 &	\bf{100.0$\pm$0.0} &   \bf{10.4$\pm$0.0}           \\
 & & & V&  		 &	98.9$\pm$0.4  &	30.2$\pm$1.5	& 99.3$\pm$0.2 &26.7$\pm$1.5	 &	\bf{99.9$\pm$0.0} &    \bf{16.8$\pm$6.7}     \\
 & & & &V			  &	99.7$\pm$0.2 &	26.2$\pm$0.9	& 85.3$\pm$1.1 & 36.8$\pm$1.0	 &	\bf{100.0$\pm$0.0} &    \bf{20.6$\pm$0.2}          \\ 
 \midrule
 \multirow{6}{*}{Lv. 2}     
& V & V& &    &         0.0$\pm$0.0  & 43.3$\pm$0.7		& 0.0$\pm$0.0 &	44.1$\pm$0.6 &	\bf{89.7$\pm$0.8} &      \bf{15.5$\pm$0.3}          \\
 & V& & V&      &         0.1$\pm$0.1  &	224.8$\pm$0.4	& 0.6$\pm$0.5 & 224.3$\pm$0.5	 &	\bf{93.9$\pm$0.7} &    \bf{ 18.8$\pm$0.3}       \\
 &V & & &  	V	 &	0.0$\pm$0.0  & 98.0$\pm$0.0	& 0.0$\pm$0.0 & 98.0$\pm$0.0	 &	\bf{95.8$\pm$0.5} &    \bf{ 32.3$\pm$0.6 }     \\
 
&&V&V&&0.4$\pm$0.1&90.8$\pm$1.3&0.2$\pm$0.2&91.4$\pm$1.1&\bf{100.0$\pm$0.0} & \bf{ 14.5$\pm$0.0 }\\ 
  & &V & &  V		 &	 0.0$\pm$0.0   &	 76.8$\pm$2.1 	&  0.0$\pm$0.0  & 79.5$\pm$1.7 	 &	\bf{ 20.0$\pm$0.0 } &    \bf{ 79.0$\pm$0.9 }     \\
 & & &V &V			  &	10.8$\pm$1.6  & 202.9$\pm$4.0 	& 10.2$\pm$2.1 & 203.2$\pm$5.1	 &	\bf{85.5$\pm$1.1} &    \bf{66.9$\pm$3.2 }          \\ 
 
 \midrule
 \multirow{4}{*}{Lv. 3}     
& V & V&V &    &         0.0$\pm$0.0  & 91.8$\pm$1.1	& 0.0$\pm$0.0 & 92.2$\pm$0.6	 &	{0.15$\pm$0.2} &    85.8$\pm$1.4          \\
 &V &V & & V     &         0.0$\pm$0.0  & 93.9$\pm$3.4	& 0.0$\pm$0.0 & 102.5$\pm$3.5	 &	{0.0$\pm$0.0} &   109.4$\pm$2.3      \\
 &V & & V&  V		 &	0.0$\pm$0.0  & 225.0$\pm$0.0	& 0.0$\pm$0.0 &  225.0$\pm$0.0 	 &	{1.6$\pm$0.6} &    {220.9$\pm$1.1 }     \\
 & &V &V &V			  &	4.3$\pm$1.0  &99.3$\pm$2.9	& 4.4$\pm$0.8 &  97.7$\pm$3.0	 &	{5.8$\pm$1.1} &   105.0$\pm$2.0         \\ 
 \midrule
 \multirow{1}{*}{Lv. 4}     
& V & V&V &  V  &          0.0$\pm$0.0   &	 96.6$\pm$8.1	 &  0.0$\pm$0.0  & 	150.5$\pm$7.5  &	{ 0.0$\pm$0.1 } &    177.2$\pm$9.2            \\
 
 
 
 
\end{tabular}
}
\caption{\qbai}
\label{tb:main}
\end{center}
\end{table*}

==> tb_all_res2.tex <==
% !TEX root = main.tex


\begin{table*}[t] 

\begin{center}
{
\begin{tabular}{c|c|cccccc}
\specialrule{.15em}{.05em}{.05em} 
                      &  & \multicolumn{2}{c}{\makecell{No Query}} & \multicolumn{2}{c}{\makecell{Query Baseline} }  & \multicolumn{2}{c}{\makecell{AFK (Ours)} } \\ \toprule\toprule
                      				&Task         & Succ.($\%$)             & Eps. Len.             & Succ.($\%$)              & Eps. Len.           & Succ.($\%$)              & Eps. Len.         \\ \hline

\multirow{4}{*}{Level 1}     
& Danger    &         60.1 $\pm$ 5.0  &		& 65.9 $\pm$ 4.8 &	 &	\bf{100.0 $\pm$ 0.0} &                \\
 & Object In Box      &         47.5 $\pm$ 2.2  &		& 51.9 $\pm$ 2.8 &	 &	\bf{100.0 $\pm$ 0.0} &           \\
 & Go to Favorite  		 &	97.9 $\pm$ 1.8  &	40.5 $\pm$ 6.0	& 99.0 $\pm$ 0.0 & 28.4 $\pm$ 2.7	 &	\bf{99.6 $\pm$ 0.1} &    \bf{16.8 $\pm$ 6.7}     \\
 & Open Door			  &	60.1 $\pm$ 5.0  &	25.8 $\pm$ 2.3	& 65.9 $\pm$ 4.8 & 97.6 $\pm$ 0.4	 &	\bf{100.0 $\pm$ 0.0} &    \bf{21.5 $\pm$ 1.2}          \\ 

\midrule
\multirow{6}{*}{Level 2}     
& Danger + Object    &         -362.73 &	-362.71	& -361.76 &	-361.55 &	\bf{-355.99} & \bf{-355.74}               \\
 & Danger + Go     &         -3943.2 & 	-3933.3 & -4025.4 & -4016.2            &      \bf{-3383.2}          &     \bf{-3381.8}            \\
 & Danger + Open  		 &	-6489.7 & -6394.3 & -6280.0 & -6222.4 & \bf{-1999.1} &	 \bf{-1977.6}              \\
 & Object + Go			  &	-20722 &	-20583 &	-21205 &	-20840 &	\bf{-11363} &	\bf{-11294}              \\ 
& Object +  Open		 &	-6489.7 & -6394.3 & -6280.0 & -6222.4 & \bf{-1999.1} &	 \bf{-1977.6}              \\
 & GO + Open			  &	-20722 &	-20583 &	-21205 &	-20840 &	\bf{-11363} &	\bf{-11294}              \\ 
\midrule
\multirow{4}{*}{Level 3}     
& Danger + Object + Go    &         -362.73 &	-362.71	& -361.76 &	-361.55 &	\bf{-355.99} & \bf{-355.74}               \\
 & Object In Box      &         -3943.2 & 	-3933.3 & -4025.4 & -4016.2            &      \bf{-3383.2}          &     \bf{-3381.8}            \\
 & Go to Favorite  		 &	-6489.7 & -6394.3 & -6280.0 & -6222.4 & \bf{-1999.1} &	 \bf{-1977.6}              \\
 & Open Door			  &	-20722 &	-20583 &	-21205 &	-20840 &	\bf{-11363} &	\bf{-11294}              \\ 
\midrule
\multirow{1}{*}{Level 4}     
& Danger    &         -362.73 &	-362.71	& -361.76 &	-361.55 &	\bf{-355.99} & \bf{-355.74}               \\


\end{tabular}
}
\caption{.}
\label{tb:main}
\end{center}
\end{table*}
